DreamFuse: Adaptive Image Fusion with Diffusion Transformer

Image fusion seeks to seamlessly integrate foreground objects with background scenes, producing realistic and harmonious fused images. Unlike existing methods that directly insert objects into the background, adaptive and interactive fusion remains a challenging yet appealing task. It requires the foreground to adjust or interact with the background context, enabling more coherent integration. To address this, we propose an iterative human-in-the-loop data generation pipeline, which leverages limited initial data with diverse textual prompts to generate fusion datasets across various scenarios and interactions, including placement, holding, wearing, and style transfer. Building on this, we introduce DreamFuse, a novel approach based on the Diffusion Transformer (DiT) model, to generate consistent and harmonious fused images with both foreground and background information. DreamFuse employs a Positional Affine mechanism to inject the size and position of the foreground into the background, enabling effective foreground-background interaction through shared attention. Furthermore, we apply Localized Direct Preference Optimization guided by human feedback to refine DreamFuse, enhancing background consistency and foreground harmony. DreamFuse achieves harmonious fusion while generalizing to text-driven attribute editing of the fused results. Experimental results demonstrate that our method outperforms state-of-the-art approaches across multiple metrics.

==> ICCV2025-Author-Kit-Feb/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> ICCV2025-Author-Kit-Feb/sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> ICCV2025-Author-Kit-Feb/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> ICCV2025-Author-Kit-Feb/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> ICCV2025-Author-Kit-Feb/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> ICCV2025-Author-Kit-Feb/sec_iccv/0_abstract.tex <==
\begin{abstract}
Image fusion seeks to seamlessly integrate foreground objects with background scenes, producing realistic and harmonious fused images. Unlike existing methods that directly insert objects into the background, adaptive and interactive fusion remains a challenging yet appealing task. It requires the foreground to adjust or interact with the background context, enabling more coherent integration. To address this, we propose an iterative human-in-the-loop data generation pipeline, which leverages limited initial data with diverse textual prompts to generate fusion datasets across various scenarios and interactions, including placement, holding, wearing, and style transfer. Building on this, we introduce DreamFuse, a novel approach based on the Diffusion Transformer (DiT) model, to generate consistent and harmonious fused images with both foreground and background information. DreamFuse employs a Positional Affine mechanism to inject the size and position of the foreground into the background, enabling effective foreground-background interaction through shared attention. Furthermore, we apply Localized Direct Preference Optimization guided by human feedback to refine DreamFuse, enhancing background consistency and foreground harmony. DreamFuse achieves harmonious fusion while generalizing to text-driven attribute editing of the fused results.
Experimental results demonstrate that our method outperforms state-of-the-art approaches across multiple metrics.
\end{abstract}

==> ICCV2025-Author-Kit-Feb/sec_iccv/1_intro.tex <==
\section{Introduction}
Foreground-background image fusion is a fundamental and practical task in image editing. Recently, with the rapid development of generation methods based on diffusion models, numerous innovative and imaginative approaches have emerged in this field. Beyond generating images purely driven by text prompts, increasing attention has been directed toward generating customized images guided by specific foreground  objects~\cite{ruiz2023dreambooth, chen2023subject, tan2024ominicontrol} or performing inpainting on designated background regions~\cite{yang2023paint} for image editing and fusion.
Going further, several methods aim to achieve harmonious fusion of foreground and background by adjusting details such as lighting~\cite{zhang2025scaling}, shadows~\cite{tarres2024thinking}, and brightness-contrast consistency~\cite{wang2023semi}, making the fused images appear more natural. Other approaches~\cite{chen2024anydoor, winter2024objectmate, he2024affordance} strive to enhance fusion by modifying the orientation, pose, or style of the foreground object while preserving its identity attributes, enabling better adaptation to the background. However, most of these methods typically focus on directly placing the foreground object into the background scene. In contrast, practical scenarios often involve more diverse and interactive cases, such as partial occlusions, alternating visibility, or interactions where the object is held, worn, or integrated into the scene.

A major challenge in handling such complex fusion scenarios is the lack of suitable datasets. Existing methods typically rely on object segmentation from images or videos~\cite{kirillov2023segment, miao2022large} followed by inpainting~\cite{rombach2022high, suvorov2022resolution} to reconstruct backgrounds. However, this multi-step process frequently suffers from quality degradation due to imprecise segmentation or suboptimal inpainting, which can introduce artifacts like shadows or residual elements in the background. Moreover, handling partially occluded foregrounds is particularly challenging~\cite{tudosiu2024mulan}, and segmentation-based data often fails to adjust object pose or perspective to align with the background during fusion.
Based on these observations, we propose an Iterative Human-in-the-Loop Data Generation Pipeline to directly generate fused data, including foregrounds, backgrounds, and the fused images, avoiding issues such as incomplete foregrounds and background artifacts. We train a DiT model on curated fused data with text prompts, modifying its attention mechanism to shared attention to ensure identity consistency across fused data. Using this model, we generate multi-scale fused data for various scenarios with diverse prompts, such as placement, handheld interactions, wearable items, logo printing, and style transfer. Throughout the process, we enhance content diversity by incorporating existing LoRA~\cite{hu2021lora} and iteratively optimize the model through manual selected data. We utilize GPT-4o to filter out low-quality fused data, such as mismatched foregrounds or degraded images, ultimately constructing a dataset of 80,000 high-quality, multi-scene, multi-scale fused image samples.

\begin{figure*}[t]
  \centering
   \includegraphics[width=0.95\linewidth]{figures/DataGeneration_Framework.pdf}
   \caption{The framework of the data generation model and position matching process. The left side of the image illustrates the design structure of our data generation model, while the right side shows the position matching process and data format. We enhance the diversity of fused data generation through flexible and rich prompts combined with various style LoRAs.}
   \label{fig:data gen}
\end{figure*}


Another critical challenge in image fusion is ensuring background consistency and foreground harmony. Some approaches~\cite{chen2024anydoor, he2024affordance} rely on masks or bounding boxes for foreground placement, blending the background outside the mask to maintain consistency. However, these approaches often fail to realistically render effects like shadows or reflections beyond the mask, limiting the realism of the fused results. Other methods~\cite{lu2023tf, wang2024primecomposer} reconstruct fused images through inversion, improving foreground harmony but often compromising background consistency.
To address this trade-off, we propose DreamFuse, an adaptive image fusion framework based on DiT. By incorporating shared attention, we condition the the fused image generation on both the foreground and background while employing positional affine to introduce the foreground's position and scale without restricting its editable regions. Additionally, we employ Localized Direct Preference Optimization (LDPO) to further optimize the foreground and background regions of the fused image, ensuring better alignment with human preferences. Experimental results demonstrate that DreamFuse performs exceptionally well across various scenarios. As shown in \cref{fig: intro}, DreamFuse produces highly realistic fusion effects for real-world images. Furthermore, during training, a certain proportion of fused image descriptions is incorporated as prompts. When given a text prompt, DreamFuse effectively responds to the input and enables attribute modifications in the fused scenes, such as turning a car into gold.


In summary, our key contributions are threefold:
\begin{itemize}
    \item We propose an iterative Human-in-the-Loop data generation pipeline and construct a comprehensive fusion dataset containing 80k diverse fusion scenarios.
    \item We propose DreamFuse, a fusion framework based on DiT, which leverages positional affine and LDPO strategies to integrate the foreground into the background more naturally and adaptively.
    \item Our method outperforms the state-of-the-art methods on various benchmarks and remains effective in real-world and out-of-distribution scenarios.
\end{itemize}

\section{Related Work}
\noindent\textbf{\textit{Customized Image Generation.}} Customized image generation aims to create user-specific images based on text prompts or reference images. Some methods~\cite{han2023svdiff, ruiz2023dreambooth, gal2022image, kumari2023multi} incorporate reference concepts into specific text prompts, while approaches~\cite{ye2023ip, zhang2024ssr, wang2024instantid} utilize additional encoders to encode reference images as visual prompts, introducing customized representations for generation. Other methods~\cite{tan2024ominicontrol, huang2024context} achieve subject-driven generation by directly concatenating reference and target images during generation. In this paper, we further extend generative diffusion models by fine-tuning on small-scale data to directly generate customized foregrounds, backgrounds, and fused images based on corresponding text prompts.



\noindent\textbf{\textit{Image Fusion.}} The goal of image fusion is to seamlessly integrate an object from a foreground image into a background image. Compared to directly cutting and pasting, some approaches~\cite{peng2024frih, zhou2024foreground, menghigh, zhang2025scaling} adjust the lighting, shadows, and colors of the pasted foreground region to achieve a more harmonious fusion. Other methods~\cite{lu2023tf, wang2024primecomposer, tao2024motioncom, winter2024objectdrop, chen2024anydoor, he2024affordance, winter2024objectmate} focus on altering the perspective, pose, or style of the foreground object to make it fit more naturally into the background image. However, these methods are often restricted to object placement. In this paper, we propose a more versatile fusion approach that supports a variety of scenarios, including hand-held objects, wearable items, and style transformations, enabling more diverse integrations.

\noindent\textbf{\textit{Human Feedback Learning.}} Many methods now leverage human feedback learning to make generated images more aligned with users’ preferences. Some approaches~\cite{xu2023imagereward, xu2024visionreward, liu2025improving} train a reward model to understand human preferences and improve the generation quality through reward feedback learning. Others~\cite{wallace2024diffusion, li2024aligning, zhang2025diffusion} utilize human comparison data to directly optimize a policy that best satisfies human preferences. For the image fusion task, we propose localized direct preference optimization, which focuses on region-specific optimization to enhance both the background consistency and the harmony in fused images.




==> ICCV2025-Author-Kit-Feb/sec_iccv/2_method.tex <==

\section{Methodology}
As shown in the data format in \cref{fig:data gen}, the image fusion task typically involves the following types of images: a foreground image $F \in \mathbb{R}^{H\times W\times 3}$ with mask $F_m \in \mathbb{R}^{H\times W}$, a background image $B \in \mathbb{R}^{H\times W\times 3}$, a fused image $I \in \mathbb{R}^{H\times W\times 3}$, a fused mask $I_m \in \mathbb{R}^{H\times W}$ associated with the fused object. The masks $F_m$ and $I_m$ are primarily used to indicate the position and size of the foreground object. In practical applications, only the centroid and bounding box of the mask are required.

\begin{figure*}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/DreamFuse_Framework.pdf}
   \caption{The framework of the DreamFuse. We apply positional affine transformations to map the foreground's position and size onto the background. The foreground and background are concatenated with the noisy fused image as condition images before DiT's attention layers. Localized direct preference optimization is then used to improve background consistency and foreground harmony.}
   \label{fig:dreamfuse}
\end{figure*}

\subsection{Iterative Human-in-the-Loop Data Generation}
\label{sec:data}
\noindent{\textbf{\textit{Data Startup.}}} Unlike methods~\cite{he2024affordance, tian2025mige} that start with a fused image to segment the foreground and generate the background using inpainting, we aim to create higher-quality fusion data with richer scenes and more diverse foreground fusion. To this end, we design an iterative, human-in-the-loop data generation process. We first extract a pair of high-quality foreground $F$ and fused image $I$ from a subject-driven dataset~\cite{tan2024ominicontrol}. 
We then manually refine the inpainting regions to remove the foreground object and its effects, such as reflections and shadows, creating a high-quality background image $B$.  A total of 86 initial samples are curated, and their corresponding descriptions $C$ are generated with GPT-4o. These data are then fed into the data generation model depicted in \cref{fig:data gen} for training.

\noindent{\textbf{\textit{Data Generation Model Design.}}} We adopt Flux~\cite{blackforest2024flux} as the base model and input our curated fusion samples $G\!=\!(F, B, I)$ with prompts $C_G\!=\!(C_F,C_B,C_I)$ in batches. 
The images and prompts are encoded into image embeddings $E_i\in \mathbb{R}^{h\times w\times d}$ and text embeddings $E_c$, supplemented by learnable tag embeddings to differentiate the foreground and background.
In Flux’s RoPE~\cite{su2024roformer} mechanism, which uses a 2D position index $P_{idx} = (i, j), \forall i \in [0, h), j \in [0, w)$ to represent image positions, we optionally introduce an offset $\Delta$ to $P_{idx}$ for $F$, $B$, and $I$ as follows: 
\begin{equation}
    P_{idx} = \left\{
    \begin{aligned}
        &(i, j), & \text{if } F, \\
        &(i, j) + \Delta, & \text{if } B, \\
        &(i, j) + 2\Delta, & \text{if } I.
    \end{aligned}
    \right.
\end{equation}
During training, adding an offset improves the model's ability to generate diverse fused scenes but performs poorly across resolutions, while omitting the offset produces overly consistent results yet adapts well to multi-scale data. Based on this, we use two models—with and without offset—to generate diverse, multi-scale samples.  Further details are provided in the supplementary materials.

To establish connections between $F$,$B$ and $I$, we modify the original independent attention mechanism in the DiT to a shared attention (SA) mechanism. As shown in \cref{fig:data gen}, after the text embeddings and image embeddings of each sample are processed through modulation and linear layers, they are concatenated to form the attention query $Q_g=[Q^c_g; Q^i_g], g\in G$, where $c$ and $i$ represent the text and image components. We then concatenate the image components of the key and value across all samples: $K_g=[K^c_g; K^i_F; K^i_B; K^i_I]$, $V_g=[V^c_g; V^i_F; V^i_B; V^i_I]$. The shared attention is then computed as:
\begin{equation}
    SA = softmax(\frac{Q_gK_g^T}{\sqrt{d}})V_g,
\end{equation}
where $d$ denotes the dimension. After applying shared attention, the model gains an initial ability to generate similar images. We then fine-tune the model with LoRA~\cite{hu2021lora} to enable the generation of high-quality image fusion samples.




\noindent{\textbf{\textit{Scene Generalizability and Style Variability.}}} Our initial data only consists of object placement scenes. After fine-tuning the data generation model, it demonstrates the ability to generalize to more diverse scene prompts. In subsequent iterations, we leverage GPT-4o with open-source prompts to generate fusion prompts $C_G$, expanding foreground objects to include animals, pets, products, portraits, and logos, while categorizing background scenes into indoor and outdoor settings. Fusion scenarios are further diversified to include placement, handheld, logo printing, wearable, and style transfer. Furthermore, we observe that the data generation model responds effectively to existing style LoRAs. Therefore, we integrate fine-tuned style LoRAs, such as depth of field, realism, and ethnicity, to further enhance fusion data in both scene variety and artistic style, mitigating the stylistic bias of the Flux base model. This expansion process is iterative: the model is fine-tuned on data generated in the previous step, additional data is generated, and high-quality fusion samples are manually curated to serve as input for the next round of fine-tuning.

\noindent{\textbf{\textit{Position Matching.}}} 
To determine the position of the foreground object in the background, we use RoMA~\cite{edstedt2024roma} to perform feature matching between the foreground and the fused image, converting the results into bounding boxes. Then we utilize SAM2~\cite{ravi2024sam} to segment the foreground object from the fused image based on these bounding boxes, yielding $I_m$. For the foreground object, we use an internal segmentation model to obtain $F_m$. The position and size of the foreground object in the background are then calculated using the centroids and bounding boxes of $I_m$ and $F_m$.



\subsection{Adaptive Image Fusion Framework}
\label{framework}
In image fusion tasks, three key aspects need to be considered: (1) how to model the relationship between the background, foreground, and fused image; (2) how to incorporate the position and size information of the foreground object into the background; (3) how to ensure background consistency and foreground harmony in the fused image.

% For the first aspect, inspired by the work of~\cite{tan2024ominicontrol}, we treat the background and foreground as conditions and the fused image as a denoised target. During attention in DiT, we concatenate the background and foreground with the noisy image embedding representing the fused image, as shown in \cref{fig:dreamfuse}. This allows information from the background and foreground to be incorporated into the fused image through attention mechanisms.
% For the second aspect, we introduce the positional information of the foreground into the background through a positional affine transformation. Finally, we design a localized direct preference optimization process that aligns the fusion network with human preferences, generating more aesthetically pleasing fused images.


\noindent\textbf{\textit{Condition-aware Modeling.}} Inspired by the work~\cite{tan2024ominicontrol}, we model the background and foreground as conditions, with the fused image treated as the denoised target. Given a fixed dataset $\mathcal{D}=\{(c_i, x_f, x_b, x_i)\}$, each sample consists of a textual description of the fused image $c_i$, along with images representing the foreground $x_f$, background $x_b$ and fused image $x_i$.
We adopt the Flux-based DiT architecture, using the foreground $x_f$  and background $x_b$ as conditions with a fix timestep $0$. Additionally, most text prompt $c_i$ are randomly dropped out with a probability $p$ during training, replaced with empty strings, while a portion of the prompts is retained to preserve the network's text-responsive capability. The DiT network is tasked with denoising the noisy fused image $x_i^t$ at timestep $t$ defined as:
\begin{equation}
    x_i^t  = (1-t)x_i + tx_n,  
\end{equation}
where $x_n\sim q(x_n)$ denotes a noise sample and $t\in[0,1]$. 
The DiT model is trained to regress the velocity field $\epsilon_\theta (x_i^t, x_f, x_b, t)$ by minimizing the Flow Matching ~\cite{lipman2022flow} objective $\mathcal{L}_{noise}(\theta)$:
\begin{equation}
    \mathbb{E}_{t,(c_i, x_f,x_b,x_i)\sim\mathcal{D},x_n\sim q(x_n)}[||\epsilon-\epsilon_\theta(c_i,x_i^t, x_f, x_b, t)||],
\end{equation}
where the target velocity field is $\epsilon=x_n-x_i$. Within the DiT attention mechanism, all components are concatenated as $[Dropout(c_i, p), x_i, x_f, x_b]$, enabling joint attention computation, as illustrated in \cref{fig:dreamfuse}.
This mechanism effectively integrates background and foreground information into the fused image through the attention layers.


\noindent\textbf{\textit{Positional Affine.}} We explore three approaches to incorporate positional information, as shown in \cref{fig:pos_affine}. The most straightforward approach is to directly transform the foreground to match the desired position and size in the background (\cref{fig:pos_affine} (b)). However, this method compresses the information of foreground during scaling, which is unfavorable for inserting small objects.
Another approach involves using the placement information of the foreground, such as the mask after positioning, as a condition. This information is encoded via a tokenizer and introduced into the attention computation (\cref{fig:pos_affine} (c)). However, this approach relies heavily on the tokenizer, requiring a large amount of data to optimize its representation of positional information.
To leverage the relative positional relationship of the foreground more directly and effectively, we propose the positional affine method shown in \cref{fig:pos_affine} (a).


Specifically, both the foreground and background are assigned 2D position index $P_{idx}^f, P_{idx}^b=(i,j), \forall i \in [0, h), j \in [0, w)$ to represent their spatial relationships within the image. When placing the foreground in a target region $P_{idx}^{r}=(u,v), \forall u \in [h_r, h_r'), v \in [w_r, w_r') $ of the background, the affine transformation matrix $A$ is computed as follows:
\begin{equation}
    A = \begin{bmatrix}
        \frac{w_r'-w_r}{w} & 0 & w_r \\
        0 & \frac{h_r'-h_r}{h} & h_r \\
        0 & 0 & 1
    \end{bmatrix}.
\end{equation}
Next, the position index $P_{idx}^r $ of the target region is mapped to the foreground with the inverse affine transformation:
\begin{equation}
    P_{idx}^{f'} = A^{-1}\begin{bmatrix}
                        u \\ v\\ 1
                    \end{bmatrix}.
\end{equation}
We utilize $P_{idx}^{f'}$ as the new position index of foreground.
By employing this positional affine transformation, and leveraging DiT's responsiveness to position index, we directly incorporate the position and size information of the foreground into the target location within the background. 
This approach eliminates the need to scale or compress the foreground, enabling a more effective and reasonable integration of positional information.

\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/DreamFuse_Pos_Affine.pdf}
   \caption{Three ways for injecting positional conditions: (a) using positional affine to map the foreground's position index to its target placement; (b) directly transforming the foreground object to the target position; (c) encoding position mask information with a tokenizer and integrating it into DiT's attention computation.}
   \label{fig:pos_affine}
\end{figure}

\noindent\textbf{\textit{Localized Preference Optimization.}} In the image fusion process, maintaining background consistency and foreground harmony is crucial. When directly generating the denoised fused image, issues such as inconsistent backgrounds or disharmonious foregrounds can easily arise. To address this, we propose Localized Direct Preference Optimization (LDPO) based on Diffusion-DPO~\cite{wallace2024diffusion, liu2025improving}, enabling the diffusion network to more effectively learn from human preferences in the context of image fusion.

We construct a dataset $\mathcal{D'}=\{(c_i, x_f, x_b, x_i^w, x_i^l )\}$ consisting of additional fused sample pairs, where $x_i^w$ aligns better with human preferences than $x_i^l$. For example, as shown in \cref{fig:dreamfuse}, $x_i^l$ can be a fused image obtained by directly copying and pasting the foreground onto the background. For simplicity, we define the model input as $x_t^{\{w,l\}}=(c_i,x_f,x_b,x_i^{t, \{w,l\}})$.
The Diffusion-DPO optimizes a policy to satisfy human preferences via objective $\mathcal{L}_{DPO}(\theta,x_t^w,x_t^l)$:
\begin{equation}
    \begin{aligned}
    \mathbb{E}\bigg[\log \sigma \Big(-\frac{\beta}{2}(||\epsilon^w-\epsilon_\theta(x_t^w,t)||^2-||\epsilon^w-\epsilon_{ref}(x_t^w,t)||^2\\
    -(||\epsilon^l-\epsilon_\theta(x_t^l,t)||^2-||\epsilon^l-\epsilon_{ref}(x_t^l,t)||^2))\Big)\bigg],
    \end{aligned}
\end{equation}
where $\epsilon_\theta(\cdot)$ and $\epsilon_{ref}(\cdot)$ denotes the predictions of optimized model and reference model, respectively, $\beta$ is the regularization coefficient and $\sigma$ is the sigmoid function. Intuitively, minimizing $\mathcal{L}_{DPO}$ encourages the predicted velocity field $\epsilon_\theta$ closer to the target velocity $\epsilon^w$ of the chosen data, while diverging from $\epsilon^l$ (the rejected data). However, not all aspects of $x_i^l$ fail to align with human preferences. For instance, in copy-paste fused images, the consistency of the background better aligns with human preferences. Therefore,  we adopt a Localized DPO strategy for $x_i^w$ and $x_i^l$. A localized foreground region $M(f)$ is defined as:
\begin{equation}
    M(f) = \left\{
    \begin{aligned}
        &1, \text{if} f\in \alpha\cdot Bbox(x_f) \\
        &0, \text{otherwise},
    \end{aligned}
    \right.
\end{equation}
where $f$ represents a pixel location, $Bbox (x_f)$ denotes the region in the bounding box of the foreground object and $\alpha$ is a dilation factor that moderately expands this region. The optimized objective $\mathcal{L}_{LDPO}(\theta, x_t^w, x_t^l, M)$ is defined as:
\begin{equation}
    \begin{aligned}
    M\cdot \mathcal{L}_{DPO}(\theta,x_t^w,x_t^l)+(1-M)\cdot \mathcal{L}_{DPO}(\theta,x_t^l,x_t^w).
    \end{aligned}
\end{equation}
We provide the pseudo-code for LDPO in the Appendix. This strategy ensures background consistency while making the foreground more harmonious and aligned with human preferences.

==> ICCV2025-Author-Kit-Feb/sec_iccv/3_exp.tex <==
\section{Experiments}


\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/vis_data_analy.pdf}
   \caption{Scene distribution of the fusion dataset, including scenario counts, indoor/outdoor background proportions, and complexity levels.}
   \label{fig:data_analy}
\end{figure}

\subsection{Dataset Analysis}
As outlined in \cref{sec:data}, we employ an iterative human-in-the-loop data generation pipeline to create approximately 400k image fusion samples. To ensure diversity, we leverage GPT-4o and existing prompt libraries during the prompt generation process to create a wide variety of prompts. After applying quality filtering techniques, including GPT-4o screening and gradient comparison, we curate a final dataset containing 80k high-quality fused image samples. We further analyze the fusion scenarios, background types, and complexity of the filtered dataset, as illustrated in \cref{fig:data_analy}. Notably, over half of the dataset features outdoor backgrounds, and approximately 23k images include hand-held scenarios. Details of the generation pipeline, quality filtering methods, and statistical results are provided in the supplementary materials.

\subsection{Implementation Details}
\noindent\textbf{Hyperparameters.}
In DreamFuse training, we adopt Flux-Dev~\cite{blackforest2024flux} as the base model. The input images are scaled proportionally from their original resolution to a short side of 512 pixels. The training procedure comprises two stages: first, the full DreamFuse 80k dataset is trained for 10k iterations with batch size 1, the Prodigy~\cite{mishchenko2023prodigy} optimizer, and a LoRA rank of 16.  Subsequently, we manually select 15k high-quality samples from the initial dataset for LDPO training. Negative samples $x_i^l$ in LDPO training consist of two types: copy-paste images and low-quality inference results generated from the selected samples after stage one. We apply the $\mathcal{L}_{LDPO}$ loss to the copy-paste data and $\mathcal{L}_{DPO}$ loss to remaining negative samples. The second stage employs the AdamW~\cite{loshchilov2017decoupled} optimizer (learning rate $5\times 10^{-5}$) for another 10k iterations. The dropout probability $p$ and dilation factor $\alpha$ is set to 99\% and 1.5. The entire training is conducted on 8 NVIDIA A100 GPUs, requiring approximately 24 hours.

\begin{table}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{5mm} % 设置列间距为 1.5mm
  \begin{tabular}{@{}l|cccc@{}}
    % \toprule
    Method & CLIP & AES & IR & VR \\
    \toprule
    ControlCom~\cite{zhang2023controlcom} & 31.28 & 6.09 & -0.27 & 1.33 \\
    TF-ICON~\cite{lu2023tf} & \textbf{32.28} & \underline{6.51} & \underline{0.266} & \underline{2.37} \\
    Anydoor~\cite{chen2024anydoor} & 31.80 & 6.27 & 0.02 & 1.31 \\
    MADD~\cite{he2024affordance} & 30.36 & 5.94 & -0.72 & 0.61 \\
    MimicBrush~\cite{chen2025zero} & 31.71 & 6.27 & -0.33 & 0.83 \\
    Ours & \underline{31.93} & \textbf{6.55} & \textbf{0.35} & \textbf{3.27} \\
    % \bottomrule
  \end{tabular}
  \caption{Quantitative evaluation results on TF-ICON dataset.}
  \label{tab:tf-icon}
\end{table}

\begin{table}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{5mm} % 设置列间距为 1.5mm
  \begin{tabular}{@{}l|cccc@{}}
    % \toprule
    Method & CLIP & AES & IR & VR \\
    \toprule
    ControlCom~\cite{zhang2023controlcom} & 34.23 & 5.76 & 0.48 & 2.20 \\
    TF-ICON~\cite{lu2023tf} & \underline{35.21} & \underline{6.06} & 0.86 & 3.88 \\
    Anydoor~\cite{chen2024anydoor} & 35.04 & 6.01 & \underline{1.01} & \underline{4.14} \\
    MADD~\cite{he2024affordance} & 33.49 & 5.66 & 0.28 & -0.08 \\
    MimicBrush~\cite{chen2025zero} & 34.46 & 6.01 & 0.56 & 3.19 \\
    Ours & \textbf{35.52} & \textbf{6.10} & \textbf{1.19} & \textbf{5.56} \\
    % \bottomrule
  \end{tabular}
  \caption{Quantitative evaluation results on  DreamFuse test dataset.}
  \label{tab:dreamfuse}
\end{table}

\noindent\textbf{Benchmarks.} We randomly selected 500 unseen samples from the generated dataset as DreamFuse test set to evaluate the model's fusion capabilities across multiple scenarios, including object placement, wearing, logo printing, handheld and style transfer. Additionally, we evaluated method's performance on out-of-domain data with the TF-ICON~\cite{lu2023tf} dataset, which consists of 332 samples spanning four visual domains: photorealism, pencil sketching, oil painting, and cartoon animation.

\noindent\textbf{Evaluation metrics.} We utilize the CLIP~\cite{radford2021learning} score to evaluate the similarity between the fused images and their corresponding descriptive texts, the AES~\cite{schuhmann2022laion} score to assess the aesthetic quality of the fused images, and the ImageReward~\cite{xu2023imagereward} (IR) score to evaluate alignment, fidelity, and harmlessness. Additionally, we employ the VisionReward~\cite{xu2024visionreward} (VR) score, which leverages a vision language model~\cite{hong2024cogvlm2} (VLM) to evaluate the fused results from multiple perspectives across various questions, better reflecting human preferences.



\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/DreamFuse_Visual_SOTA.pdf}
   \caption{Qualitative comparisons with existing methods. The first row is from the TF-ICON dataset, while the others are from the DreamFuse test set.  Our approach achieves a more seamless integration of foreground objects with the background images, resulting in higher visual consistency and realism.}
   \label{fig:sota_qualitative}
\end{figure}


\subsection{Comparisons with Existing Methods}

\noindent\textbf{Quantitative results.} We evaluate several existing state-of-the-art image fusion methods on the TF-ICON and DreamFuse test datasets, including image composition methods such as TF-ICON~\cite{lu2023tf}, Anydoor~\cite{chen2024anydoor}, MADD~\cite{he2024affordance} and ControlCom~\cite{zhang2023controlcom}, as well as the reference-based fusion method MimicBrush~\cite{chen2025zero} . As shown in \cref{tab:tf-icon}, our method outperforms existing approaches across multiple metrics on the TF-ICON dataset, with a notable 0.9 improvement in the VR score compared to the second-best method. The TF-ICON contains both realistic images and images from diverse domain, and our results highlight the robustness and generalization capability of our approach. Similarly, as shown in \cref{tab:dreamfuse}, our method achieves superior performance on the DreamFuse test set, surpassing the second-best method by 1.4. Our method consistently demonstrates better fusion quality across all scenarios.

\noindent\textbf{Qualitative results.} \cref{fig:sota_qualitative} presents the qualitative visualization results of our method compared with other methods. As shown, our method not only performs well across various fusion scenarios but also excels when the fused foreground object contains reflective surfaces. 
Specifically, for elements like the mirror in the last row, DreamFuse can perceive the surrounding environment and adaptively adjust the reflections on the mirror, resulting in more natural fusion image. Detailed discussions on fusion effects in real-world scenarios are provided in the supplementary materials.

\noindent\textbf{User study.} As shown in \cref{fig:user_study}, we randomly select 200 samples and conduct a user study with 17 participants to compare our method with Anydoor~\cite{chen2024anydoor} and TF-ICON~\cite{lu2023tf}. The evaluation focus on three perspectives: the consistency of the fused image’s foreground and background with the input, the harmony of the fusion image, and the overall fusion quality. The results demonstrate that our method outperforms existing approaches across all three dimensions, achieving a 64.6\% score in overall fusion quality.

\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/vis_user_study.pdf}
   \caption{User Study: Evaluation from three perspectives: consistency, harmony, and overall quality.}
   \label{fig:user_study}
\end{figure}


\begin{table}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{5mm} % 设置列间距为 1.5mm
  \begin{tabular}{@{}l|cccc@{}}
    % \toprule
    Method & CLIP & AES & IR & VR \\
    \toprule
    Direct Trans. & 35.04 & 6.10 & 0.98 & 4.72 \\
    Mask Token. & 35.14 & 6.11 & 1.03 & 4.93 \\
    Pos. Affine & \textbf{35.22} & \textbf{6.13} & \textbf{1.07} & \textbf{5.28} \\
    % \bottomrule
  \end{tabular}
  \caption{Qualitative analysis of three positional incorporation strategies on the DreamFuse test set after the first-stage training.}
  \label{tab:ab-pos-affine}
\end{table}


\subsection{Ablation Study}
\noindent\textbf{Positional affine.} We compare the three positional incorporation strategies discussed in \cref{framework}. As shown in \cref{tab:ab-pos-affine}, the results on the DreamFuse test set after the first-stage training demonstrate that the positional affine approach achieves the highest CLIP and VR scores, reaching 35.215 and 5.278, respectively. This suggests that the positional affine method better preserves the information of foreground objects, outperforming the direct transform and mask tokenizer strategies, which are more prone to information loss of fine-grained details.

\begin{table}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{3mm} % 设置列间距为 1.5mm
  \begin{tabular}{@{}l|cccc@{}}
    % \toprule
    DreamFuse & CLIP & AES & IR & VR \\
    \toprule
    First-Stage Training & 35.22 & \textbf{6.13} & 1.07 & 5.28 \\
    w/ $\mathcal{L}_{DPO}$ & 35.36 & 6.07 & 1.16 & 5.52 \\
    w/ $\mathcal{L}_{DPO}$ + $\mathcal{L}_{LDPO}$  & 35.51 & 6.10 & 1.17 & \textbf{5.58} \\
    w/ $\mathcal{L}_{DPO}$ + $\mathcal{L}_{LDPO} + \mathcal{L}_{noise}$ & \textbf{35.52} & 6.10 & \textbf{1.19} & 5.56 \\
    % \bottomrule
  \end{tabular}
  \caption{Qualitative analysis of localized preference optimization.}
  \label{tab:ab_ldpo}
\end{table}



\noindent\textbf{Localized preference optimization.} In the second stage of training, we employ Localized Direct Preference Optimization (LDPO) to further enhance the model's performance by utilizing two types of paired data: the first type consists of poorly performing and well-performing results generated after the first training stage with different seeds and optimized with the $\mathcal{L}_{DPO}$, while the second type involves copy-paste data treated as negative samples and optimized with the $\mathcal{L}_{LDPO}$. As shown in \cref{tab:ab_ldpo}, ``$w/\ \mathcal{L}_{DPO}$'' refers to training with only the first type of data, ``$w/\ \mathcal{L}_{LDPO}$'' refers to training with copy-pasted data. Results indicate the LDPO significantly improves fusion performance by achieving an approximate 0.11 increase in IR scores compared to the first-stage results. Further incorporating the $\mathcal{L}{noise}$ loss results in a comparable performance. LDPO primarily enhances background consistency and foreground harmony, as visually demonstrated in \cref{fig:ab_ldpo}, where using copy-paste data as negative samples allows the model to better capture fusion-related transformations, such as perspective and affine adjustments, rather than simply copying and pasting the foreground, while also improving the consistency of other background regions.

\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{figures/DreamFuse_Visual_LDPO.pdf}
   \caption{Qualitative results about the LDPO. Compared to ``$w/\ \mathcal{L}_{DPO}$'', ``$w/\ \mathcal{L}_{LDPO}$'' leverages copy-paste data to better help the model understand perspective changes in the foreground while maintaining background consistency as much as possible.}
   \label{fig:ab_ldpo}
\end{figure}

\noindent\textbf{Dropout probability $p$.} To retain the diffusion model's text response capability, allowing it to edit the fused foreground based on the prompt, we include the fusion image's text as a prompt at a dropout probability $p$. However, we find that when the dropout probability is set too low, such as 80\%, the model's response to empty text weakens, resulting in the inability to properly integrate the foreground into the background. As shown in \cref{fig:Dropout probability} (a), lower dropout probabilities lead to lower CLIP scores for the fusion results, indicating that the foreground is not well integrated into the background. Therefore, we ultimately chose $p=99\%$, which preserves the model's text response capability to a greater extent without compromising its performance.
\begin{figure}[t]
  \centering
  \includegraphics[width=0.49\linewidth]{figures/visual_prompt_ratio.pdf} 
  \includegraphics[width=0.49\linewidth]{figures/visual_alpha.pdf}
   \caption{The effectiveness about the dropout probability $p$ and dilation factor $\alpha$.}
   \label{fig:Dropout probability}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/DreamFuse_Visual_car.pdf}
   \caption{The responsiveness to different prompts.}
   \label{fig:car}
\end{figure}

\noindent\textbf{Dilation factor $\alpha$.} Intuitively, the dilation factor $\alpha$ defines the size of the local harmonious region around the foreground considered during the LDPO process.  As shown in \cref{fig:Dropout probability} (b), we investigate the impact of $\alpha$ on the model's performance. When $\alpha=1$, the model focuses solely on the harmony within the bounding box of the object, disregarding external factors such as shadows or reflections, which are then treated as non-preferred, leading to a performance drop. When $\alpha=0$, copy-paste data is entirely treated as samples consistent with human preferences, resulting in a significant decline in the VR score. As $\alpha$ increases, the preference for background consistency gradually diminishes, though it has minimal impact on overall harmony. Based on these findings, we set $\alpha=1.5$ for LDPO training.

\noindent\textbf{Responsiveness to text prompts.} In our experiments, we find that DreamFuse responds effectively to text prompts without additional training. This enables modifications to the attributes of foreground objects or the fusion scene, as shown in \cref{fig:car}.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1\linewidth]{figures/visual_alpha.pdf}
%    \caption{The effectiveness about the dilation factor $\alpha$.}
%    \label{fig:Dilation factor}
% \end{figure}


\subsection{Conclusion}
In this paper, we first propose an iterative human-in-the-loop data generation pipeline to create fusion scenarios that are relatively rare in traditional fusion tasks, making the fusion process more natural and flexible. Using this pipeline, we generated a dataset of 80k fusion data that encompass various scenarios, including placement, handheld, wearable, and style transfer tasks. Additionally, we introduce DreamFuse, an adaptive image fusion framework with the diffusion transformer. This framework incorporates positional affine transformations to encode the position and size of foreground, employs shared attention mechanisms to establish connections between the foreground and background, and ultimately leverages localized direct preference optimization to further enhance the quality of the fused images. Experimental results show that our method outperforms existing approaches on multiple benchmarks.
